TEMPO: A Realistic Multi-Domain Benchmark for Temporal Reasoning-Intensive Retrieval

Existing temporal QA benchmarks focus on simple fact-seeking queries from news corpora, while reasoning-intensive retrieval benchmarks lack temporal grounding. However, real-world information needs often require reasoning about temporal evolution and synthesizing evidence across time periods. We introduce TEMPO, the first benchmark combining temporal reasoning with reasoning-intensive retrieval across 13 domains. TEMPO features: (1) 1,730 complex queries requiring deep temporal reasoning such as tracking changes, identifying trends, or comparing cross-period evidence; (2) step-wise retrieval planning with 3,976 decomposed steps and gold documents mapped to each step for multi-hop evaluation; and (3) novel temporal metrics including Temporal Coverage@k and Temporal Precision@k measuring whether results span required time periods. Evaluation of 12 retrieval systems reveals substantial challenges: the best model (DiVeR) achieves only 32.0 NDCG@10 and 71.4\% Temporal Coverage@10, demonstrating difficulty in retrieving temporally complete evidence. We believe TEMPO provides a challenging benchmark for improving temporal reasoning in retrieval and RAG systems. Our code and data are available at https://github.com/tempo-bench/Tempo. See also our official website: https://tempo-bench.github.io/.

==> latex_ablation/main_ablation_variants.tex <==
\begin{table*}[t]
\centering
\caption{Ablation study on query variants. NDCG@10 averaged across all domains. Best in \textbf{bold}, second best \underline{underlined}. Baseline uses original queries; Strip removes temporal signals; Temporal-Only retains only temporal information; Normalized adds explicit temporal intent tags.}
\label{tab:ablation_variants}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{Baseline} & \textbf{Strip} & \textbf{Temporal-Only} & \textbf{Normalized} & \textbf{$\Delta$ (Base-Strip)} \\
\midrule
\rowcolor{gray!12}\multicolumn{6}{c}{\textit{Sparse}} \\
\midrule
BM25 & 10.8 & 10.4 & 11.0 & 10.9 & +0.4 \\
\midrule
\rowcolor{gray!12}\multicolumn{6}{c}{\textit{Dense (<1B)}} \\
\midrule
BGE & 22.0 & 19.5 & 9.6 & 22.1 & +2.5 \\
Contriever & 21.4 & 18.9 & 10.2 & 22.4 & +2.5 \\
Inst-L & 24.8 & 23.2 & 13.5 & 24.7 & +1.6 \\
SBERT & 24.9 & 23.3 & 8.7 & 23.5 & +1.6 \\
\midrule
\rowcolor{gray!12}\multicolumn{6}{c}{\textit{Dense (>1B)}} \\
\midrule
E5 & \underline{30.4} & 27.0 & 14.2 & 29.1 & +3.4 \\
GritLM & 27.2 & 24.9 & 15.2 & 27.1 & +2.4 \\
Qwen & 22.8 & 21.2 & \underline{17.2} & 23.3 & +1.6 \\
SFR & 30.0 & \underline{27.8} & 16.3 & 29.5 & +2.2 \\
\midrule
\rowcolor{gray!12}\multicolumn{6}{c}{\textit{Reasoning}} \\
\midrule
DiVeR & \textbf{32.0} & \textbf{29.9} & \textbf{17.7} & \underline{30.2} & +2.1 \\
Rader & 24.2 & 21.8 & 9.4 & 21.6 & +2.4 \\
ReasonIR & 27.3 & 25.1 & 13.8 & \textbf{35.3} & +2.1 \\
\midrule
\bottomrule
\end{tabular}}
\end{table*}

==> latex_tables/main_temporal_metrics.tex <==
\begin{table}[t]
\centering
\caption{Temporal metrics@10 averaged across all domains. Best in \textbf{bold}, second best \underline{underlined}.}
\label{tab:temporal_avg_metrics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{TP@10} & \textbf{TR@10} & \textbf{TC@10} & \textbf{NDCG|FC@10} \\
\midrule
BM25 & 24.0 & 11.1 & 32.8 & 22.5 \\
BGE & 53.7 & 34.0 & 66.1 & 25.3 \\
Contriever & 49.6 & 30.3 & 64.1 & 26.2 \\
DiVeR & \textbf{62.0} & \textbf{41.3} & \underline{71.4} & \underline{32.5} \\
E5 & 53.5 & 31.1 & 63.2 & \textbf{33.4} \\
GritLM & 53.8 & 35.0 & 69.1 & 27.2 \\
Inst-L & 53.1 & 33.8 & 66.9 & 25.8 \\
Qwen & 46.2 & 28.8 & 61.0 & 29.9 \\
Rader & 50.6 & 32.3 & 66.1 & 26.1 \\
ReasonIR & \underline{57.4} & \underline{38.2} & \textbf{72.4} & 28.8 \\
SBERT & 54.1 & 35.0 & 67.2 & 26.9 \\
\bottomrule
\end{tabular}}
\end{table}
